Measurement of D0-anti-D0 Mixing using the Ratio of Lifetimes for the Decays D0 --> K-pi+, K-K+, and pi-pi+

We present a measurement of $D^0$-$\bar{D^0}$ mixing parameters using the ratios of lifetimes extracted from a sample of $D^0$ mesons produced through the process $D^{*+}\to\D^0\pi^+$, that decay to $K^{+}\pi^{-}$, K^{-}K^{+}$, or $\pi^-\pi^+$. The Cabibbo-suppressed modes $K^{-}K^{+}$ and $\pi^-\pi^+$ are compared to the Cabibbo-favored mode $K^{+}\pi^{-}$ to obtain a measurement of $y_{CP}$, which in the limit of CP conservation corresponds to the mixing parameter $y$. The analysis is based on a data sample of 384 $fb^{-1}$ collected by the $BaBar$ detector at the PEP-II asymmetric-energy $e^+e^-$ collider. We obtain $y_{CP} = [1.24\pm 0.39\mathrm{(stat)} \pm 0.13\mathrm{(syst)}]%$, which is evidence of $D^0$-$\bar{D^0}$ mixing at the $3\sigma$ level, and $\Delta Y = [-0.26\pm 0.36\mathrm{(stat)} \pm 0.08 \mathrm{(syst)}]%$, where $\Delta Y$ constrains possible CP violation. Combining this result with a previous $BaBar$ measurement of $y_{CP}$ obtained from a separate sample of $D^0\to K^{-}K^{+}$ events, we obtain $y_{CP} = [1.03\pm 0.33 \mathrm{(stat)} \pm 0.19 \mathrm{(syst)}]%$.

==> abstract.tex <==
We present a measurement of $D^0$-$\overline{D^0}$ mixing parameters using the ratios of
lifetimes extracted from a sample of $D^0$ mesons produced through the process
$D^{*+}\rightarrow\D^0\pi^+$, that decay to $K^{+}\pi^{-}$,
$K^{-}K^{+}$, or $\pi^-\pi^+$. The Cabibbo-suppressed modes $K^{-}K^{+}$ and $\pi^-\pi^+$ are
compared to the Cabibbo-favored mode $K^{+}\pi^{-}$ to obtain a measurement
of $y_{CP}$, which in the limit of $CP$ conservation corresponds to
the mixing parameter $y$. 
The analysis is based on a data sample of 384~$fb^{-1}$
collected by the $BaBar$ detector at the PEP-II asymmetric-energy
$e^+e^-$ collider. We obtain
$  y_{CP}     =  [1.24\pm 0.39\mathrm{(stat)} \pm 0.13\mathrm{(syst)}]\%$, which is evidence
of $D^0$-$\overline{D^0}$ mixing at the $3\sigma$ level, and $\Delta Y  =  [-0.26\pm
0.36\mathrm{(stat)} \pm 0.08\mathrm{(syst)}]\%$, where $\Delta Y$ constrains possible $CP$ violation.
Combining this result with a previous $BaBar$ measurement of $y_{CP}$
obtained from a separate sample
of $D^0\rightarrow K^{-}K^{+}$ events, we obtain
$  y_{CP}     =  [1.03\pm 0.33\mathrm{(stat)} \pm 0.19 \mathrm{(syst)}]\%$.



==> babarsym.tex <==
%%%%%   Standard symbols for use in BABAR papers and BAD Notes
%%%%%
%%%%%   Revised   05/22/01 P. Dauncey     Added \hepex, etc. and clean up a bit
%%%%%   Revised   12/07/00 D. Hitlin      Added features of D. Kirkby's HEP.sty
%%%%%   Revised   07/13/00 R. Waldi       Corrected \Kbar, \Bbar ... macros
%%%%%   Revised   07/13/00 D. MacFarlane  Replaced incorrect \chic1 symbols
%%%%%   Revised   07/05/00 P. Dauncey     Added \mes, \mec, removed \O
%%%%%   Revised   07/04/00 D. MacFarlane  Added scalable version of BABAR
%%%%%   Revised   07/01/00 D. MacFarlane
%%%%%   Revised   06/21/00 D. Hitlin
%%%%%   Original  06/10/00 D. Hitlin
%%%%%   Revision of TDR and Physics Book symbol file
%%%%%

\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% BABAR ... THE NAME OF THE COLLABORATION %%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^-\pi^+}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}

% Obsolete
\newcommand{\dstr}{\ensuremath{\Dstar}\xspace}
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace}
\newcommand{\dsp}{\ensuremath{\Dstarp}\xspace}
\newcommand{\dsm}{\ensuremath{\Dstarm}\xspace}
\newcommand{\dsz}{\ensuremath{\Dstarz}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}

% added by GHM on March 25, 2003 -- from Andrei Gritsan
\def\BorBbar    {\kern 0.18em\optbar{\kern -0.18em B}{}\xspace}
\def\DorDbar    {\kern 0.18em\optbar{\kern -0.18em D}{}\xspace}
\def\KorKbar    {\kern 0.18em\optbar{\kern -0.18em K}{}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\def\chicJ  {\ensuremath{\chi_{cJ}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% TAU BRANCHING FRACTIONS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR         {{\ensuremath{\cal B}\xspace}}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}\xspace}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}\xspace}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}\xspace}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  LIGHT HADRON DECAYS %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}\xspace}
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  B DECAYS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}\xspace}
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}\xspace}
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}\xspace}
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}\xspace}
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}\xspace}
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}\xspace}
\def\bupsik     {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}\xspace}
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}\xspace}

\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}\xspace}
\def\Bzbtox     {\ensuremath{\Bzb \to \X}\xspace}
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}\xspace}
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}\xspace}
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}\xspace}
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}\xspace}
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}\xspace}
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}\xspace}
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}\xspace}
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}\xspace}
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}\xspace}
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}\xspace}

\def\BtoDK      {\ensuremath{B \to DK}\xspace}
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}\xspace}
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}\xspace}
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}\xspace}
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}\xspace}

\def\Btoetah    {\ensuremath{B \to \eta h}\xspace}
\def\Btoetaph   {\ensuremath{B \to \etapr h}\xspace}

\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}\xspace}
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}\xspace}

\def\btosgam    {\ensuremath{b \to s \g}\xspace}
\def\btodgam    {\ensuremath{b \to d \g}\xspace}
\def\btosll     {\ensuremath{b \to s \ellell}\xspace}
\def\btosnunu   {\ensuremath{b \to s \nunub}\xspace}
\def\btosgaga   {\ensuremath{b \to s \gaga}\xspace}
\def\btosglue   {\ensuremath{b \to s g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  Y(4S) DECAYS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace}
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}\xspace}
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}\xspace}
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  TAU DECAYS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}\xspace}
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}\xspace}
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}\xspace}
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}\xspace}
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}\xspace}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GAMMA-GAMMA REACTIONS %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ggtopi     {\ensuremath{\gaga \to \pipi}\xspace}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}\xspace}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}\xspace}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\rm t}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\mec        {\mbox{$m_{\rm EC}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}
%\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
%\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}} 
%\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}} 
%\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}} 
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}} 
%\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}} 
%\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}} 
%\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}} 
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}} 
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}} 
%\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}} 
%\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
%\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
%\def\mum  {\ensuremath{{\rm \,\mum}}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 
%\def\muma {\ensuremath{\rm \,\mum}^2\xspace}
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees


%\def\m          {\ensuremath{\rm \,m}}    %% meter
%\def\ma         {\ensuremath{\rm \,m}^2}  %% meter squared
%\def\cm         {\ensuremath{\rm \,cm}}   %% centimeter
%\def\cma        {\ensuremath{\rm \,cm}^2} %% centimeter squared
\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}
%\def\mm         {\ensuremath{\rm \,mm}}   %% millimeter
%\def\mma        {\ensuremath{\rm \,mm}^2} %% millimeter squared
%\def\mum        {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma       {\ensuremath{\,\mu\rm m^2}}


\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

%\renewcommand{\bar}[1]{\overline{#1}}  

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}


\def\pep2{PEP-II}
\def\BF{$B$-Factory}
\def\abf {asymmetric \BF}
\def\sx    {\ensuremath{\sigma_x}\xspace}     
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}


\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}


% Data processing
\def\kbytes     {\ensuremath{{\rm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\rm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}\xspace}
%




% QCD parameters

\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{%
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace
}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}


% CKM, CP violation

\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
%\def\CPT               {\ensuremath{C\!P\!T}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!
% added by GHM on March 25, 2003
\def\C       {\ensuremath{C}\xspace}
\def\P       {\ensuremath{P}\xspace}
\def\T       {\ensuremath{T}\xspace}



\def\epstag  {\ensuremath{\varepsilon_{\rm tag}}\xspace}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}}, 
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|, 
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\cal D}\xspace}
\def\deltaz{\ensuremath{{\rm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}




% Journal References

% These bases are useful for ``submitted to'' when no volume is needed
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
%\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
%\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.\xspace}
%\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods\xspace}
%\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
%\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Meth.\xspace}
% update the following based on input from John Ripka, Asst. Editor at PRL, August 2006
\newcommand{\nimBaseA}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ A\xspace}
\newcommand{\nimBaseB}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ B\xspace}
\newcommand{\nimBaseC}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ C\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ D\xspace}
\newcommand{\nimBaseE}       {Nucl.\ Instrum.\ Methods Phys.\ Res., Sect.\ E\xspace}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\zpBase}         {Z.\ Phys.\xspace}


\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\bf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\bf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\bf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instrum.\ and Methods~{\bf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimaa}       [1]  {\nimBaseE~{\bf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instrum.\ Methods~{\bf A{\bf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseA~{\bf #1}}
\newcommand{\nimb}      [1]  {\nimBaseB~{\bf #1}}
\newcommand{\nimc}      [1]  {\nimBaseC~{\bf #1}}
\newcommand{\nimd}      [1]  {\nimBaseD~{\bf #1}}
\newcommand{\nime}      [1]  {\nimBaseE~{\bf #1}}
% add commands for NIM articles from earlier periods
% for NIM articles from 1981-1983
\newcommand{\oldnim}    [1]  {Nucl.\ Instrum.\ Methods Phys.\ Res.~{\bf #1}}
% for NIM articles prior to 1981
\newcommand{\oldernim}  [1]  {Nucl.\ Instrum.\ Methods~{\bf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\bf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\bf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\bf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\bf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\bf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\bf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Theor.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\bf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\bf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}


%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}\xspace}
\def\bbsim      {\mbox{\tt BBsim}\xspace}
\def\beast      {\mbox{\tt Beast}\xspace}
\def\beget      {\mbox{\tt Beget}\xspace}
\def\Bta        {\mbox{\tt Beta}\xspace}
\def\betakfit   {\mbox{\tt BetaKfit}\xspace}
\def\cornelius  {\mbox{\tt Cornelius}\xspace}
\def\evtgen     {\mbox{\tt EvtGen}\xspace}
\def\euclid     {\mbox{\tt Euclid}\xspace}
\def\fitver     {\mbox{\tt FitVer}\xspace}
\def\fluka      {\mbox{\tt Fluka}\xspace}
\def\fortran    {\mbox{\tt Fortran}\xspace}
\def\gcalor     {\mbox{\tt GCalor}\xspace}
\def\geant      {\mbox{\tt GEANT}\xspace}
\def\gheisha    {\mbox{\tt Gheisha}\xspace}
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace}
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}\xspace}
\def\minuit     {\mbox{\tt Minuit}\xspace}
\def\objegs     {\mbox{\tt Objegs}\xspace}
\def\paw        {\mbox{\tt Paw}\xspace}
\def\Root       {\mbox{\tt Root}\xspace}
\def\squaw      {\mbox{\tt Squaw}\xspace}
\def\stdhep     {\mbox{\tt StdHep}\xspace}
\def\trackerr   {\mbox{\tt TrackErr}\xspace}
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% version number
%
\def\version    {\ensuremath{6}\xspace}

\def\CPV        {\ensuremath{C\!P\!V}\xspace}
%
% additional software packages
%
\def\kkf           {\mbox{{\cal KK}}\xspace}
\def\geantiv       {\mbox{\tt GEANT 4}\xspace}
\def\jetsetvii     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
\def\pythiavvii    {\mbox{\tt Pythia \hspace{-0.5em}5.\hspace{-0.2em}7}\xspace}
% 
% cos(thetaDzCm)
%
%\def\thetaDzCm    {\ensuremath{\theta^*_{\Dz}}\xspace}
\def\thetaDzCm     {\ensuremath{\theta_{\rm CM}}\xspace}
\def\costhetaDzCm  {\ensuremath{\cos\thetaDzCm}\xspace}
\def\Ndz           {\ensuremath{N_{\rm RS+}}\xspace}
\def\Ndzb          {\ensuremath{N_{\rm RS-}}\xspace}
\def\RDzDzb        {\ensuremath{R_{\rm RS+/RS-}}\xspace}
\def\RDzDzbGen     {\ensuremath{R^{\rm gen}_{\rm RS+/RS-}}\xspace}
\def\AsyFB         {\ensuremath{A_{\c\cbar}}\xspace}
%
% skim name
%
\def\DzSkim     {\hbox{\tt D0To2ProngDcj}}
%
% D-mixing- and D-lifetime-specific symbols for BAD 1291.
%
%\def\Rdcs       {\ensuremath{R_{\rm DCS}}\xspace}
\def\Rdcs       {\ensuremath{R_{\rm D}}\xspace} % BaBar doesn't like 
                                                % multi-letter subscripts.
\def\RdcsPM     {\ensuremath{R_{\rm D}^{\pm}}\xspace}
\def\RdcsP      {\ensuremath{R_{\rm D}^{+}}\xspace}
\def\RdcsM      {\ensuremath{R_{\rm D}^{-}}\xspace}
\def\Rpm        {\ensuremath{R^{\pm}}\xspace}
\def\Rws        {\ensuremath{R_{\rm WS}}\xspace}
\def\RwsO       {\ensuremath{R^{O}_{\rm WS}}\xspace}
\def\RwsOp      {\ensuremath{R^{O+}_{\rm WS}}\xspace}
\def\RwsOm      {\ensuremath{R^{O-}_{\rm WS}}\xspace}
\def\RwsT       {\ensuremath{R_{\rm WS}}\xspace}
\def\RwsTp      {\ensuremath{R^{+}_{\rm WS}}\xspace}
\def\RwsTm      {\ensuremath{R^{-}_{\rm WS}}\xspace}
\def\Rm         {\ensuremath{R_{\rm M}}\xspace}
\def\RmPm       {\ensuremath{R_{\rm M}^{\pm}}\xspace}
\def\RmP        {\ensuremath{R_{\rm M}^{+}}\xspace}
\def\RmM        {\ensuremath{R_{\rm M}^{-}}\xspace}
\def\xPrimeSq   {\ensuremath{{x^{\prime}}^2}\xspace}
\def\yPrimeSq   {\ensuremath{{y^{\prime}}^2}\xspace}
\def\xPrime     {\ensuremath{x^{\prime}}\xspace}
\def\xPrimeP    {\ensuremath{x^{\prime+}}\xspace}
\def\xPrimeM    {\ensuremath{x^{\prime-}}\xspace}
\def\yPrime     {\ensuremath{y^{\prime}}\xspace}
\def\yPrimeP    {\ensuremath{y^{\prime+}}\xspace}
\def\yPrimeM    {\ensuremath{y^{\prime-}}\xspace}
\def\xPrimePmSq {\ensuremath{{x^{\prime\pm}}^2}\xspace}
\def\xPrimeParenPmSq {\ensuremath{{x^{\prime(\pm)}}^2}\xspace}
\def\yPrimePmSq {\ensuremath{{y^{\prime\pm}}^2}\xspace}
\def\xPrimePm   {\ensuremath{x^{\prime\pm}}\xspace}
\def\yPrimePm   {\ensuremath{y^{\prime\pm}}\xspace}
\def\yPrimeParenPm   {\ensuremath{y^{\prime(\pm)}}\xspace}
\def\xPrimePSq  {\ensuremath{{x^{\prime+}}^2}\xspace}
\def\xPrimeMSq  {\ensuremath{{x^{\prime-}}^2}\xspace}
\def\AwsT       {\ensuremath{A_{\rm WS}}\xspace}
\def\Aws        {\ensuremath{A^O_{\rm WS}}\xspace}
\def\AD         {\ensuremath{A_{\rm D}}\xspace}
\def\AM         {\ensuremath{A_{\rm M}}\xspace}
\def\ADPDG      {\ensuremath{A_{\rm D}^{\rm PDG}}\xspace}
\def\AMPDG      {\ensuremath{A_{\rm M}^{\rm PDG}}\xspace}
\def\pisoft     {\ensuremath{\pi_{\rm s}}\xspace}
\def\pisoftp    {\ensuremath{\pi_{\rm s}^{+}}\xspace}
\def\pisoftm    {\ensuremath{\pi_{\rm s}^{-}}\xspace}
\def\st         {\ensuremath{\sigma_{t}}\xspace}
\def\qOp        {\ensuremath{\left|\frac{p}{q}\right|}\xspace}
%
% mixing parameter symbols
%
\def\bone       {\ensuremath{b_1}}
\def\btwo       {\ensuremath{b_2}}
\def\bthree     {\ensuremath{b_3}}
\def\bonep       {\ensuremath{b_1^+}}
\def\btwop       {\ensuremath{b_2^+}}
\def\bthreep     {\ensuremath{b_3^+}}
\def\bonem       {\ensuremath{b_1^-}}
\def\btwom       {\ensuremath{b_2^-}}
\def\bthreem     {\ensuremath{b_3^-}}
\def\bonepm       {\ensuremath{b_1^\pm}}
\def\btwopm       {\ensuremath{b_2^\pm}}
\def\bthreepm     {\ensuremath{b_3^\pm}}
\def\btwonew       {\ensuremath{\tilde{b}_2}}
\def\bthreenew     {\ensuremath{\tilde{b}_3}}

%
% Symbols from BAD 251.
%
\def\Dztopipi   {\ensuremath{\Dz \to \pi^{+}\pi^{-}}\xspace}
\def\Dztokk     {\ensuremath{\Dz \to K^{+}K^{-}}\xspace}
\def\Dztokpi    {\ensuremath{\Dz \to K^{-}\pi^{+}}\xspace}
\def\DztoKPi    {\ensuremath{\Dz \to K\pi}\xspace}
\def\Dzbtokpi   {\ensuremath{\Dzb \to K^{+}\pi^{-}}\xspace}
\def\DztokpiWS  {\ensuremath{\Dz \to K^{+}\pi^{-}}\xspace}
\def\DzbtokpiWS {\ensuremath{\Dzb \to K^{-}\pi^{+}}\xspace}
\def\Kppim      {\ensuremath{K^{+}\pi^{-}}\xspace}
\def\Kmpip      {\ensuremath{K^{-}\pi^{+}}\xspace}
\def\KmKp       {\ensuremath{K^{-}K^{+}}\xspace}
\def\KpKm       {\ensuremath{K^{+}K^{-}}\xspace}
\def\pimpip     {\ensuremath{\pi^{-}\pi^{+}}\xspace}
\def\pippim     {\ensuremath{\pi^{+}\pi^{-}}\xspace}
\def\mKpiPre    {\ensuremath{m_{K\pi}^{\hbox{pre}}}\xspace}
\def\mDz        {\ensuremath{m_{\Dz}}\xspace}
\def\mDst       {\ensuremath{m_{\Dstar}}\xspace}
\def\mDstp      {\ensuremath{m_{{\Dstar}^+}}\xspace}
\def\mDsp       {\ensuremath{m_{\dsp}}\xspace}
\def\m          {\ensuremath{M}\xspace}
\def\mb         {\ensuremath{\overline{{M}^{0}}}\xspace}
\def\leb        {\ensuremath{\left<\right.}}
\def\reb        {\ensuremath{\left>\right.}}
\def\eb         {\ensuremath{\left|\right.}}
\def\egm        {\ensuremath{\eb\m\reb}\xspace}
\def\emb        {\ensuremath{\eb\mb\reb}\xspace}
\def\mge        {\ensuremath{\leb\m\eb}\xspace}
\def\mbe        {\ensuremath{\leb\mb\eb}\xspace}
\def\micron     {\ensuremath{\mu}m\xspace}
\def\mhh        {\ensuremath{m_{h^+h^{\prime-}}}}
\newcommand{\kevcc}{\ensuremath{{\mathrm{\,Ke\kern -0.1em V\!/}c^2}}\xspace}
%
% Monte Carlo samples
%
\def\uds        {\ensuremath{uds}}
\def\tauptaum   {\ensuremath{\tau^+\tau^-}}
%
% independent variables
%
\def\mKpi       {\ensuremath{m_{K\pi}}\xspace}
\def\dm         {\ensuremath{\Delta m}\xspace}
\def\t          {\ensuremath{t}}
\def\terr       {\ensuremath{\sigma_{\t}}\xspace}
%
% subsystem TLA
%
\def\svt         {\ensuremath{{\rm SVT}}}
\def\dch         {\ensuremath{{\rm DCH}}}
\def\drc         {\ensuremath{{\rm DRC}}}
\def\emc         {\ensuremath{{\rm EMC}}}
\def\ifr         {\ensuremath{{\rm IFR}}}
%
% mathematical symbols
%
%\def\chisq       {\ensuremath{\chi^2}}
\def\Pchisq      {\ensuremath{P(\chi^2)}}
\def\PchisqDz    {\ensuremath{P(\chi^2_{\Dz})}}
\def\PchisqDst   {\ensuremath{P(\chi^2_{\Dstar})}}
\def\erf         {\ensuremath{{\rm erf}}}
%
% normalization constants
%
\def\CG          {\ensuremath{C_{\rm G}}\xspace}     % Gaussian
\def\CJSU        {\ensuremath{C_{\rm JSU}}\xspace}   % Johnson-SU
\def\CCG         {\ensuremath{C_{\rm CG}}\xspace}    % Correlated Gaussian
\def\CA          {\ensuremath{C_{\rm T}}\xspace}     % reverse Argus 
\def\CCB         {\ensuremath{C_{\rm CB}}\xspace}     % reverse Argus 
%
% luminosity values
%
\def\lumitotnum  {\ensuremath{383.83}}
\def\lumitot     {\ensuremath{\lumitotnum\invfb}}
\def\lumionnum   {\ensuremath{347.23}}
\def\lumion      {\ensuremath{\lumionnum\invfb}}
\def\lumioffnum  {\ensuremath{36.60}}
\def\lumioff     {\ensuremath{\lumioffnum\invfb}}
\def\lumin       {\ensuremath{\mathcal{L}}}
\def\lumifb      {\ensuremath{\mathcal{L}\;[\invfb]}} 
%
% Dstar and slow pi
%
\def\Dst         {\ensuremath{D^{*}}}
\def\Dstp        {\ensuremath{D^{*+}}}
\def\Dstm        {\ensuremath{D^{*-}}}
\def\slowpi      {\ensuremath{\pi_s}}
\def\slowpip     {\ensuremath{\slowpi^+}}
\def\slowpim     {\ensuremath{\slowpi^-}}
%
% efficiency symbols
%
\def\ekmpip      {\ensuremath{\epsilon_{\Km\pip}}}
\def\ekppim      {\ensuremath{\epsilon_{\Km\pim}}}
\def\effRS       {\ensuremath{\epsilon_{\rm RS}}}
\def\effWS       {\ensuremath{\epsilon_{\rm WS}}}
\def\effratav    {\ensuremath{R_{\overline{\epsilon}}}\xspace}
\def\effratp     {\ensuremath{R_\epsilon^+}\xspace}
\def\effratm     {\ensuremath{R_\epsilon^-}\xspace}
\def\deffratav   {\ensuremath{\delta\effratav}\xspace}
\def\effrat      {\ensuremath{R_\epsilon}\xspace}
%
% kinematic quantities
%
\def\plabslowpi  {\ensuremath{p_{\pisoft}}}
\def\nsvtslowpi  {\ensuremath{N^{\svt}_{\pisoft}}}
\def\ndchslowpi  {\ensuremath{N^{\dch}_{\pisoft}}}
\def\ndchdz      {\ensuremath{N^{\dch}_{K,\pi}}}
\def\pstar       {\ensuremath{p^*}}
\def\pstarDz     {\ensuremath{\pstar_{\Dz}}}
\def\pstarSlowPi {\ensuremath{\pstar_{\slowpi}}}
\def\psec        {\ensuremath{{\rm \,psec}}\xspace}  %% picosecond
\def\fsec        {\ensuremath{{\rm \,fsec}}\xspace}  %% femtosecond
%
% DOCAs
%
\def\rdoca       {\ensuremath{R_{\rm DOCA}}\xspace}
\def\zdoca       {\ensuremath{z_{\rm DOCA}}\xspace}
%
% D0 related symbols
%
\def\mDkpi      {\ensuremath{m_{k\pi}}}
%
% list/category symnbols
%
%\def\DstarTagged    {\hbox{\tt DstarTagged}\xspace}
%\def\DzUntagged     {\hbox{\tt D0Untagged}\xspace}
%\def\KpiTagged      {\hbox{\tt KpiTagged}\xspace}
%\def\KpiTaggedRS    {\hbox{\tt KpiTaggedRS}\xspace}
%\def\KpiTaggedWS    {\hbox{\tt KpiTaggedWS}\xspace}
%\def\KKTagged       {\hbox{\tt KKTagged}\xspace}
%\def\pipiTagged     {\hbox{\tt pipiTagged}\xspace}
%\def\KpiUntagged    {\hbox{\tt KpiUnTagged}\xspace}
%\def\KKUnTagged     {\hbox{\tt KKTagged}\xspace}
\def\TwoBodyAnal    {\hbox{\tt TwoBodyAnal}\xspace}
\def\SlmPdfBuilder  {\hbox{\tt SlmPdfBuilder}\xspace}
\def\TwoBodyApp     {\hbox{\tt TwoBodyApp}\xspace}
\def\TwoBodyUserApp {\hbox{\tt TwoBodyUserApp}\xspace}
\def\catone         {\hbox{\tt category 1}\xspace}
\def\cattwo         {\hbox{\tt category 2}\xspace}
\def\catthree       {\hbox{\tt category 3}\xspace}
\def\catfour        {\hbox{\tt category 4}\xspace}
\def\Cascade        {\hbox{\tt Cascade}\xspace}
\def\TreeFitter     {\hbox{\tt TreeFitter}\xspace}
%
% RS, WS symbols
%
\def\RightSign      {{Right Sign}\xspace}
\def\rightsign      {{right sign}\xspace}
\def\WrongSign      {{Wrong Sign}\xspace}
\def\wrongsign      {{wrong sign}\xspace}

%
% category yields
%
\def\niRS         {\ensuremath{N_{1{\rm RS}}}\xspace}
\def\niWS         {\ensuremath{N_{1{\rm WS}}}\xspace}
\def\niiRS        {\ensuremath{N_{2{\rm RS}}}\xspace}
\def\niiWS        {\ensuremath{N_{2{\rm WS}}}\xspace}
\def\niiiRS       {\ensuremath{N_{3{\rm RS}}}\xspace}
\def\niiiWS       {\ensuremath{N_{3{\rm WS}}}\xspace}
\def\nivRS        {\ensuremath{N_{4{\rm RS}}}\xspace}
\def\nivWS        {\ensuremath{N_{4{\rm WS}}}\xspace}
\def\nDzRS        {\ensuremath{N_{{\rm RS}}^{+}}\xspace}
\def\nDzbRS       {\ensuremath{N_{{\rm RS}}^{-}}\xspace}
\def\nDzWS        {\ensuremath{N_{{\rm WS}}^{+}}\xspace}
\def\nDzbWS       {\ensuremath{N_{{\rm WS}}^{-}}\xspace}
\def\nDzRST       {\ensuremath{N_{{\rm RS}}^{T+}}\xspace}
\def\nDzbRST      {\ensuremath{N_{{\rm RS}}^{T-}}\xspace}
\def\nDzWST       {\ensuremath{N_{{\rm WS}}^{T+}}\xspace}
\def\nDzbWST      {\ensuremath{N_{{\rm WS}}^{T-}}\xspace}
\def\effDzRS      {\ensuremath{\epsilon_{{\rm RS}}^{+}}\xspace}
\def\effDzbRS     {\ensuremath{\epsilon_{{\rm RS}}^{-}}\xspace}
\def\effDzWS      {\ensuremath{\epsilon_{{\rm WS}}^{+}}\xspace}
\def\effDzbWS     {\ensuremath{\epsilon_{{\rm WS}}^{-}}\xspace}

%
% Poisson pull quantities
%
\def\Nobsi{\ensuremath{N^{\rm obs}_i}}
\def\Npdfi{\ensuremath{N^{\rm pdf}_i}}

% 
% decay time fit symbols
%
\def\RmyPrime {\ensuremath{(\Rm, \yPrime)}\xspace}
\def\decayt {\ensuremath{t}}
\def\ttrue  {\ensuremath{t_{\rm true}}\xspace}
%\def\terr   {\ensuremath{\sigma \t}\xspace}
\def\toff   {\ensuremath{t_0}\xspace}
\def\like   {\ensuremath{{\cal L}}}
\def\likelife {\ensuremath{\like_{\tau}}\xspace}
\def\likemix  {\ensuremath{\like_{mix}}\xspace}
\def\liketoff  {\ensuremath{\like_{\toff}}\xspace}
\def\liketoffz {\ensuremath{\like_{\toff=0}}\xspace}
\def\likerat  {\ensuremath{\Lambda}\xspace}
\def\dLL      {\ensuremath{\Delta \rm LL}\xspace}
\def\dNLL#1{\ensuremath{\Delta {\rm NLL}(#1)}\xspace}
\def\tlife    {\ensuremath{\tau}}
% Don't put spaces after the `#1' in the next line, it will cause the
% macro to absorb tokens into argument 1 up to the next blank space
\def\TwsFull#1{\ensuremath{T_{\rm WS}(#1;\bone,\btwo,\bthree,\tau)}}
\def\Tws  {\ensuremath{T_{\rm WS}(t)}}
\def\TwsPM{\ensuremath{T_{\rm WS}^{\pm}(t)}}
%
% PDF symbols
%
\def\res{\ensuremath{{\cal R}}}
\def\mdmnospace            {\ensuremath{(\mKpi,\,\dm)}}
\def\mdm            {\mdmnospace\xspace}
\def\mdmt            {\ensuremath{(\mKpi,\,\dm,\,t)}\xspace}
\def\mdmtdt          {\ensuremath{(\mKpi,\,\dm,\,\decayt,\,\terr)}\xspace}
\def\xpsqyp          {\ensuremath{(\xPrimeSq,\,\yPrime)}\xspace}
%\def\xpyp            {\ensuremath{(\xPrime,\,\yPrime)}\xspace}
\def\Swapped {\ensuremath{{\cal P}_{swapK\pi}}\xspace}
\def\Gauss#1{\ensuremath{G{#1}}\xspace}
\def\Jsu#1{\ensuremath{J_{\rm SU#1}}\xspace}
\def\CB#1{\ensuremath{CB_{\rm #1}}\xspace}
\def\Gcorr{\ensuremath{G_{\rm corr}}\xspace}
%\def\Psignal{\ensuremath{{\cal S}}\xspace}
\def\Psignal{\ensuremath{{\cal P}_1}\xspace}
\def\Swide{\ensuremath{{\cal P}_{\rm wide}}\xspace}
\def\SJsu{\ensuremath{{\cal P}_{\Jsu{}}}\xspace}
\def\Score{\ensuremath{{\cal P}_{\rm core}}\xspace}
\def\Siicore{\ensuremath{{\cal P}_{2\rm core}}\xspace}
%\def\FmKpiPeakingBkg{\ensuremath{{\cal F}}\xspace}
\def\FmKpiPeakingBkg{\ensuremath{{\cal P}_2}\xspace}
%\def\FmKpiPeakingBkgRS{\ensuremath{{\cal F}_{\rm RS}}\xspace}
\def\FmKpiPeakingBkgRS{\ensuremath{{\cal P}_{\rm 2RS}}\xspace}
%\def\FmKpiPeakingBkgWS{\ensuremath{{\cal F}_{\rm WS}}\xspace}
\def\FmKpiPeakingBkgWS{\ensuremath{{\cal P}_{\rm 2WS}}\xspace}
%\def\BDeltaMPeakingBkgRS{\ensuremath{{\cal B}_{\rm RS}}\xspace}
\def\BDeltaMPeakingBkgRS{\ensuremath{{\cal P}_{\rm 3RS}}\xspace}
%\def\BDeltaMPeakingBkgWS{\ensuremath{{\cal B}_{\rm WS}}\xspace}
\def\BDeltaMPeakingBkgWS{\ensuremath{{\cal P}_{\rm 3WS}}\xspace}
%\def\CNonPkgBkgRS{\ensuremath{{\cal C}_{\rm RS}}\xspace}
\def\CNonPkgBkgRS{\ensuremath{{\cal P}_{\rm 4RS}}\xspace}
%\def\CNonPkgBkgWS{\ensuremath{{\cal C}_{\rm WS}}\xspace}
\def\CNonPkgBkgWS{\ensuremath{{\cal P}_{\rm 4WS}}\xspace}
\def\poly#1{\ensuremath{{P_{#1}}}\xspace}
\def\polyicatiiiWS{\ensuremath{p_{1}^{\rm cat3WS}}\xspace}
\def\polyiicatiiiWS{\ensuremath{p_{2}^{\rm cat3WS}}\xspace}
\def\polyicativRS{\ensuremath{p_{1}^{\rm cat4RS}}\xspace}
\def\polyiicativRS{\ensuremath{p_{2}^{\rm cat4RS}}\xspace}
\def\polyicativWS{\ensuremath{p_{1}^{\rm cat4WS}}\xspace}
\def\polyiicativWS{\ensuremath{p_{2}^{\rm cat4WS}}\xspace}

%
% swapped kpi PDF symbols
%
\def\CSWAPPOLY    {\ensuremath{C_{\rm swap}}\xspace}
\def\mswap        {\ensuremath{m_{\rm swap}}\xspace}

\def\xbar{\ensuremath{\overline x}\xspace} 
\def\xbari{\ensuremath{{\overline x}_i}\xspace}
\def\sigmai{\ensuremath{\sigma_i}\xspace}
\def\sigmaxi{\ensuremath{\sigma_{x,i}}\xspace}
\def\ybar{\ensuremath{\overline y}\xspace}
\def\ybari{\ensuremath{{\overline y}_{i}}\xspace}
\def\sigmayi{\ensuremath{\sigma_{y,i}}\xspace}
\def\kcorr{\ensuremath{k_{\rm corr}}\xspace}
\def\Argus#1{\ensuremath{A_{\rm #1}}\xspace}
%\def\kcutoff{\ensuremath{k_{\rm cutoff}}\xspace}
\def\kcutoff{\ensuremath{\dm_{\rm min}}\xspace}
%\def\kslope{\ensuremath{k_{\rm slope}}\xspace}
%\def\kslopei#1{\ensuremath{k_{{\rm slope},{#1}}}\xspace}
\def\kslopei#1{\ensuremath{\dm^{\rm {#1}}_{\rm slope}}\xspace}
\def\kslope{\ensuremath{\dm_{\rm slope}}\xspace}
%\def\kslopecatii{\ensuremath{k_{\rm cat2}}\xspace}
\def\kslopecatii{\kslopei{cat2}}
%\def\kslopecatiiRS{\ensuremath{k_{\rm cat2RS}}\xspace}
\def\kslopecatiiRS{\kslopei{cat2RS}}
%\def\kslopecatiiWS{\ensuremath{k_{\rm cat2WS}}\xspace}
\def\kslopecatiiWS{\kslopei{cat2WS}}
%\def\kslopecatiiiRS{\ensuremath{k_{\rm cat3RS}}\xspace}
\def\kslopecatiiiRS{\kslopei{cat3RS}}
%\def\kslopecatiiiWS{\ensuremath{k_{\rm cat3WS}}\xspace}
\def\kslopecatiiiWS{\kslopei{cat3WS}}
%\def\kslopecativRS{\ensuremath{k_{\rm cat4RS}}\xspace}
\def\kslopecativRS{\kslopei{cat4RS}}
%\def\kslopecativWS{\ensuremath{k_{\rm cat4WS}}\xspace}
\def\kslopecativWS{\kslopei{cat4WS}}
%\def\kcutoffi#1{\ensuremath{k_{{\rm cutoff},{#1}}}\xspace}
\def\kcutoffi#1{\ensuremath{\dm_{{\rm min},{#1}}}\xspace}

\def\mGi{\ensuremath{\overline{m}_{1}}\xspace}
\def\mGii{\ensuremath{\overline{m}_{2}}\xspace}
\def\mGiii{\ensuremath{\overline{m}_{3}}\xspace}
\def\sigGi{\ensuremath{\sigma_{m_1}}\xspace}
\def\sigGii{\ensuremath{\sigma_{m_2}}\xspace}
\def\sigGiii{\ensuremath{\sigma_{m_3}}\xspace}

\def\mCG{\ensuremath{\overline{m}_{\rm {CG}}}\xspace}
\def\sigCG{\ensuremath{\sigma_{{m_{\rm CG}}}}\xspace}
\def\dmCG{\ensuremath{\overline{\dm}_{\rm CG}}\xspace}
\def\dmsigCG{\ensuremath{\sigma_{\dm_{\rm CG}}}\xspace}

\def\mCGiii{\ensuremath{\overline{m}_{\rm {CG3}}}\xspace}
\def\sigCGiii{\ensuremath{\sigma_{{m_{\rm CG3}}}}\xspace}
\def\dmCGiii{\ensuremath{\overline{\dm}_{\rm CG3}}\xspace}
\def\dmsigCGiii{\ensuremath{\sigma_{\dm_{\rm CG3}}}\xspace}
\def\kcorriii{\ensuremath{k_{\rm correl3}}\xspace}

\def\ficore{\ensuremath{f_{\rm 1{\rm core}}}\xspace}
\def\fiiicore{\ensuremath{f_{\rm 3{\rm core}}}\xspace}

\def\dmGi{\ensuremath{\overline{\dm}_{\rm {1}}}\xspace}
\def\dmGii{\ensuremath{\overline{\dm}_{\rm {2}}}\xspace}
\def\dmGiii{\ensuremath{\overline{\dm}_{\rm {3}}}\xspace}
\def\dmsigGi{\ensuremath{\sigma_{\dm_{1}}}\xspace}
\def\dmsigGii{\ensuremath{\sigma_{\dm_{2}}}\xspace} 
\def\dmsigGiii{\ensuremath{\sigma_{\dm_{3}}}\xspace} 

\def\dmJSU{\ensuremath{\overline{\dm}_{J_{\rm SU}}}\xspace}
\def\dmsigJSU{\ensuremath{\sigma_{J_{\rm SU}}^{\dm}}\xspace}
\def\fJSU{\ensuremath{f_{J_{\rm SU}}}\xspace}

\def\dmcatiiiRS{\ensuremath{\overline{\dm}_{\rm cat3WS}}\xspace}
\def\dmsigcatiiiRS{\ensuremath{\sigma_{\rm cat3WS}}\xspace}
%\def\dmcatiiiWS{\ensuremath{\overline{\dm}_{\rm cat3WS}}\xspace}
%\def\dmsigcatiiiWS{\ensuremath{\sigma_{\rm cat3WS}}\xspace}

\def\fwide{\ensuremath{f_{\rm wide}}\xspace}

\def\mCGm{\ensuremath{m_{\rm CG_{\mKpi}}}\xspace} 
\def\mCGdm{\ensuremath{m_{\rm CG_{\dm}}}\xspace}
\def\sigCGm{\ensuremath{\sigma_{\rm CG_{\mKpi}}}\xspace}
\def\sigCGdm{\ensuremath{\sigma_{{\rm CG}_{\dm}}}\xspace}
\def\correl{\ensuremath{k_{\rm correl}}\xspace} 

\def\RterrSig{\ensuremath{H_{\terr}^{\rm sig}}\xspace} 
\def\RterrBkg{\ensuremath{H_{\terr}^{\rm bkg}}\xspace} 

%
% Rws fit variation labels
%
\def\defaultVar{Default fit}
\def\catiPDFVar{Cat.~1 PDF}
\def\catiiPDFVar{Cat.~2 PDF}
\def\nCatiiiRSVar{Cat.~3 RS yield}
\def\catiiiRSVar{Cat.~3 RS shape}
\def\catiiiWSPDFVar{Cat.~3 WS PDF}
\def\cativRSPDFVar{Cat.~4 RS PDF}
\def\terrTightVar{\ensuremath{0<\terr<0.4\psec}}
\def\terrLooseVar{\ensuremath{0<\terr<0.6\psec}}
\def\terrVar{\terr criterion}
%\def\adjudicationVar{Adjudication criterion}
\def\keepOverlapsVar{Keep all overlapping candidates}
\def\rejectOverlapsVar{Remove all overlapping candidates}

% Rws values
%
\def\dRws#1{\ensuremath{\delta R_{\rm WS}^{\rm #1}}\xspace}
\def\RwsData{\ensuremath{0.3533}}
\def\RwsDataStat{\ensuremath{0.0080}}
\def\RwsDataSigSyst{\ensuremath{0.487}}
\def\RwsDataSyst{\ensuremath{0.0039}}
\def\RwsRbMC{\ensuremath{0.3990}}
\def\RwsRbMCStat{\ensuremath{0.0076}}
\def\RwsRbMCSigSyst{\ensuremath{0.780}}
\def\RwsRbMCSyst{\ensuremath{0.0059}}
\def\RwsRaMC{\ensuremath{0.3977}}
\def\RwsRaMCStat{\ensuremath{0.0086}}
\def\RwsRaMCSigSyst{\ensuremath{0.690}}
\def\RwsRaMCSyst{\ensuremath{0.0059}}
%
% lifetime, mixing systematics
%
\def\tauSyst{\ensuremath{\delta\tau^{\rm syst}}\xspace}
\def\yPrimeSyst{\ensuremath{\delta y^{\prime\rm syst}}\xspace}
\def\RmSyst{\ensuremath{\delta\Rm^{\rm syst}}\xspace}
\def\RdcsSyst{\ensuremath{\delta\Rdcs^{\rm syst}}\xspace}
\def\cdesw{1.40in}
%
% blinded caveat
%
\def\blinded{{\rm \bf The mixing parameter values are currently blinded.}}

% 
% Macros for general discussion of mixing and CPV phenomenology.
%
\def\Pbar    {\ensuremath{\kern 0.2em\overline{\kern -0.2em P}{}}\xspace}
\def\Pz      {\ensuremath{P^0}\xspace}
\def\Pzb     {\ensuremath{\Pbar^0}\xspace}
\def\ketPz   {\ensuremath{|\Pz\rangle}\xspace}
\def\ketPzb  {\ensuremath{|\Pzb\rangle}\xspace}
\def\Pzphys  {\ensuremath{P^0_{\rm phys}(t)}\xspace}
\def\Pzbphys {\ensuremath{\Pbar^0_{\rm phys}(t)}\xspace}
\def\ketPzphys {\ensuremath{|P^0_{\rm phys}(t)\rangle}\xspace}
\def\ketPzbphys{\ensuremath{|\Pbar^0_{\rm phys}(t)\rangle}\xspace}
\def\ketPL   {\ensuremath{|P_{\rm L}\rangle}\xspace}
\def\ketPH   {\ensuremath{|P_{\rm H}\rangle}\xspace}
\def\ketPi   {\ensuremath{|P_1\rangle}\xspace}
\def\ketPii  {\ensuremath{|P_2\rangle}\xspace}
\def\pL      {\ensuremath{p_{\rm L}}\xspace}
\def\pH      {\ensuremath{p_{\rm H}}\xspace}
\def\pone    {\ensuremath{p_1}\xspace}  % Can't override \pi 
\def\ptwo    {\ensuremath{p_2}\xspace}
\def\qL      {\ensuremath{q_{\rm L}}\xspace}
\def\qH      {\ensuremath{q_{\rm H}}\xspace}
\def\qi      {\ensuremath{q_1}\xspace}
\def\qii     {\ensuremath{q_2}\xspace}
\def\braPz   {\ensuremath{\langle\Pz|}\xspace}
\def\braPzb  {\ensuremath{\langle\Pzb|}\xspace}
\def\f       {\ensuremath{f}\xspace}
\def\fbar    {\ensuremath{\overline{f}}\xspace}
\def\ketf    {\ensuremath{|\f\rangle}\xspace}
\def\ketfbar {\ensuremath{|\fbar\rangle}\xspace}
\def\braf    {\ensuremath{\langle\f|}\xspace}
\def\brafbar {\ensuremath{\langle\fbar|}\xspace}
\def\A       {\ensuremath{A}\xspace}
\def\Abar    {\ensuremath{\overline{A}}\xspace}
\def\Af      {\ensuremath{A_{\f}}\xspace}
\def\myAfb   {\ensuremath{A_{\fbar}}\xspace}
\def\Abfb    {\ensuremath{{\overline{A}}_{\fbar}}\xspace}
\def\Abf     {\ensuremath{{\overline{A}}_{\f}}\xspace}
\def\H       {\ensuremath{H}\xspace}
\def\Hz      {\ensuremath{H_0}\xspace}
\def\Hstrong {\ensuremath{H_{\rm strong}}\xspace}
\def\Hem     {\ensuremath{H_{\rm EM}}\xspace}
\def\Hw      {\ensuremath{H_{\rm W}}\xspace}
\def\ketpsi#1{\ensuremath{|\psi(#1)\rangle}\xspace}
\def\M       {\ensuremath{M}\xspace}
\def\MH      {\ensuremath{M_{\rm H}}\xspace}
\def\ML      {\ensuremath{M_{\rm L}}\xspace}
\def\G       {\ensuremath{\Gamma}\xspace}
\def\GH      {\ensuremath{\Gamma_{\rm H}}\xspace}
\def\GL      {\ensuremath{\Gamma_{\rm L}}\xspace}
%\def\Dm      {\ensuremath{\Delta m}\xspace}  % Already defined above for reco
                                              % mass diff
\def\DM      {\ensuremath{\Delta M}\xspace}   % Use this for D mass splitting
\def\DG      {\ensuremath{\Delta\Gamma}\xspace}
\def\Di      {\ensuremath{D_1}\xspace}
\def\Dii     {\ensuremath{D_2}\xspace}
\def\Mi      {\ensuremath{M_1}\xspace}
\def\Mii     {\ensuremath{M_2}\xspace}
\def\Gi      {\ensuremath{\Gamma_1}\xspace}
\def\Gii     {\ensuremath{\Gamma_2}\xspace}
\def\lf      {\ensuremath{\lambda_{\f}}\xspace}
\def\lbf     {\ensuremath{\overline{\lambda}_{\f}}\xspace}
\def\lbfb    {\ensuremath{\overline{\lambda}_{\fbar}}\xspace}
\def\lfb     {\ensuremath{\lambda_{\fbar}}\xspace}

%
% significance (-2 delta LL/2.3)
%
\def\signif  {\ensuremath{{\cal s}^2}\xspace}
%
% macro for tables
%
\def\lbox#1#2{\setbox1=\hbox{\parbox{#1}{\raggedright #2}}\vrule width0pt height1.2\ht1 depth1.5\dp1\box1}

\def\cbox#1#2{\setbox1=\hbox{\parbox{#1}{\raggedright\centering #2}}\vrule width0pt height1.2\ht1 depth1.5\dp1\box1}

%
%  Macro \dk: for particle decay chains.  Example:
%
%    \begin{eqnarray*}
%    \Dstarp & \to & \pip \Dz \\
%    &&\phantom{\pip}\dk \Km \pip  
%    \end{eqnarray*}
%
% Uses '\phantom{}' to place the decay arrow under the decaying particle.
%
\catcode`\@=11\relax
\newskip\dkwidth
\def\dk{%
   \dkwidth=2em plus 0.5 em minus 0.25 em\relax
   {\m@th\mathord{%
   \hbox{%
      \kern 0.3em%  Changed from 0.4.  RFC 861003.
      \raise 0.6ex%
      \hbox{%
         \vrule width 0.25pt height 0.5\dkwidth depth0pt}%
      \kern-1.2pt%
      \hbox to 1.1\dkwidth{% 
         \rightarrowfill}%
      \kern0.4em}}%
   }%
}%
%
%  MOD RFC 861003  Change the spacing between the `-' and the \leaders
%                  in \rightarrowfill from -6mu to -10mu to prevent
%                  a gap from occuring there.
%
\def\rightarrowfill{$\m@th\mathord-\mkern-10mu%
  \cleaders\hbox{$\mkern-2mu\mathord-\mkern-2mu$}\hfill
  \mkern-6mu\mathord\rightarrow$}
%
\catcode`\@=12\relax
%
% misc mathematical symbols
%
\def\Cov#1#2{\ensuremath{\hbox{cov}({#1},{#2})}\xspace}
\def\cov#1{\Cov{#1}{#1}}
\def\corr#1#2{\ensuremath{\hbox{corr}({#1},{#2})}\xspace}
%
%
%
\def\yCP        {\ensuremath{y_{C\!P}}\xspace}
\def\yCPkk      {\ensuremath{y_{C\!P}^{KK}}\xspace}
\def\yCPpipi    {\ensuremath{y_{C\!P}^{\pi\pi}}\xspace}
\def\deltaY     {\ensuremath{\Delta Y}\xspace}
\def\deltaYkk   {\ensuremath{\Delta Y^{KK}}\xspace}
\def\deltaYpipi {\ensuremath{\Delta Y^{\pi\pi}}\xspace}
\def\Kmpip      {\ensuremath{\Km\pip}\xspace}
\def\pimpip     {\ensuremath{\pim\pip}\xspace}
\def\tauKpi     {\ensuremath{\tau_{K\pi}}\xspace}
\def\tauhh      {\ensuremath{\tau_{hh}}\xspace}
\def\tauhhp     {\ensuremath{\tau_{hh}^+}\xspace}
\def\tauhhm     {\ensuremath{\tau_{hh}^-}\xspace}
\def\tauKK      {\ensuremath{\tau_{KK}}\xspace}
\def\tauKKp     {\ensuremath{\tau_{KK}^+}\xspace}
\def\tauKKm     {\ensuremath{\tau_{KK}^-}\xspace}
\def\taupipi    {\ensuremath{\tau_{\pi\pi}}\xspace}
\def\taupipip   {\ensuremath{\tau_{\pi\pi}^+}\xspace}
\def\taupipim   {\ensuremath{\tau_{\pi\pi}^-}\xspace}
\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}

